Variational Autoencoding of PDE Inverse Problems

Specifying a governing physical model in the presence of missing physics and recovering its parameters are two intertwined and fundamental problems in science. Modern machine learning allows one to circumvent these, via emulators and surrogates, but in doing so disregards prior knowledge and physical laws that are especially important for small data regimes, interpretability, and decision making. In this work we fold the mechanistic model into a flexible data-driven surrogate to arrive at a physically structured decoder network. This provides accelerated inference for the Bayesian inverse problem, and can act as a drop-in regulariser that encodes a-priori physical information. We employ the variational form of the PDE problem and introduce stochastic local approximations as a form of model based data augmentation. We demonstrate both the accuracy and increased computational efficiency of the framework on real world settings and structured spatial processes.

==> Impact/theo_comment.tex <==
\theo{This needs rewriting. Take a step back and list in your head or on notes all the possible ways this work can have positive and negative impact. You have good material in there now but needs fleshing out with a bit more structure. See also advice online on writing the impact statement. Here is some more specific ideas:
\begin{itemize}
    \item Use it smartly to highlight all the novelty and contributions of the work again: why uncertainty over mech is important and what are the implications? Interpretability and why its important nowadays and what it leads to? Scalability of the approach and what it means in terms of applying it to various areas in engineeirng and industry? Methodological impact (you do cover that a bit) like opening up new avenues of research for Phi-ML and Uncertainty Quantification. 
    \item Impact from environmental applications like the ones you demonstrate. What does it mean to better estimate ground water depth? or pollution/contamination? social good?
    \item Impact in engineering and physics sciences/domains. Ease of plugin means ease of adoption and areas of engineering requireing massive FEMs and massive compute. If you are also saving compute resources you are also reducing carbon footprint of FEM analysis that is happening across most of engineeirng industry. 
    \item Use a citation or two to support your above impact claims by citing something that reviews the history of FEM and its industry impact. Not sure if this is relevant: \textit{A BRIEF HISTORY OF THE BEGINNING OF THE FINITE ELEMENT METHOD
K. K. GUPTA  J. L. MEEK}
    \item Look at these and similar FEM adoption links: \url{https://innovationatwork.ieee.org/the-advantages-of-fem/} and \url{https://www.digitalengineering247.com/article/structural-fea-in-the-automotive-industry/} and \url{https://www.simscale.com/blog/2015/11/75-years-of-the-finite-element-method-fem/}
    \item{Does your mini-patching enables federated learning/distributed approaches, some divide and conquer style approach or map-reduce approach for FEM? That can be huge}
    \item{FEM has a huge industry. From wikipedia: ``The finite element method (FEM) is the most widely used method for solving problems of engineering and mathematical models."}
\end{itemize}
}
